Completeness for Prime-Dimensional Phase-Affine Circuits

Equational reasoning about circuits underpins quantum-circuit optimisation and verification. In the qubit CNOT-dihedral fragment, phase polynomials and layered normal forms support a complete equational theory. We develop the corresponding theory for prime-dimensional qudits, where basis labels, value controls, and phase exponents share prime-field arithmetic. We first describe reversible affine circuits over F_d as transformations x -> Ax + b, with an affine normal form extending Lafont's linear normal form by translations. Adjoining finite-angle diagonal phases by polynomial degree yields linear, quadratic, and cubic calculi. Their binomial-basis identities expose the mixed diagonal gates forced by affine transport. These calculi have unique phase-affine normal forms, and the resulting equational theories are complete: semantic equality coincides with derivable equality.

==> eptcsdata.tex <==
\providecommand{\firstpage}{40}
\providecommand{\publicationstatus}{J. van de Wetering, O. Oreshkov, and A.B. Sainz (Eds.):\\
Quantum Physics and Logic 2026 (QPL 2026)\\
EPTCS 456, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.456.3}{10.4204/EPTCS.456.3}}
\pdfoutput=1


==> figuremap.tex <==
\makeatletter
\newcommand{\qplmap}[4]{%
  \expandafter\def\csname qplfig@#1\endcsname{{#2}{#3}{#4}}%
  \expandafter\def\csname qplfig@./#1\endcsname{{#2}{#3}{#4}}}
\newcommand{\qplinclude}[3]{%
  \raisebox{-#3}{%
    \includegraphics[page=#2,pagebox=mediabox]{#1}}}
\newcommand{\qplfigure}[1]{%
  \ifcsname qplfig@#1\endcsname
    \begingroup
    \edef\qplentry{\csname qplfig@#1\endcsname}%
    \expandafter\qplinclude\qplentry
    \endgroup
  \else
    \PackageError{eptcsfigures}{Missing precompiled figure `#1'}{}%
  \fi}
\newcommand{\tikzfig}[1]{\qplfigure{#1}}
\newcommand{\qcfig}[1]{\qplfigure{#1}}
\qplmap{axioms/AxiomCXX}{atlas/figures01.pdf}{1}{13.96504pt}
\qplmap{axioms/AxiomCXXtop}{atlas/figures01.pdf}{2}{13.96504pt}
\qplmap{axioms/AxiomMult1}{atlas/figures01.pdf}{3}{3.66437pt}
\qplmap{axioms/AxiomMultCNOT2A}{atlas/figures01.pdf}{4}{8.84354pt}
\qplmap{axioms/AxiomMultCNOT2A-00}{atlas/figures01.pdf}{5}{8.84354pt}
\qplmap{axioms/AxiomMultCNOT2A-01}{atlas/figures01.pdf}{6}{8.84354pt}
\qplmap{axioms/AxiomMultCNOT2B}{atlas/figures01.pdf}{7}{8.84354pt}
\qplmap{axioms/AxiomMultCNOTA}{atlas/figures01.pdf}{8}{13.96504pt}
\qplmap{axioms/AxiomMultCNOTB}{atlas/figures01.pdf}{9}{13.96504pt}
\qplmap{axioms/AxiomMultCNOTtwisted2A}{atlas/figures01.pdf}{10}{13.96504pt}
\qplmap{axioms/AxiomMultCNOTtwisted2B}{atlas/figures01.pdf}{11}{13.62277pt}
\qplmap{axioms/AxiomMultXMultY}{atlas/figures01.pdf}{12}{3.66437pt}
\qplmap{axioms/AxiomMultXY}{atlas/figures01.pdf}{13}{3.66437pt}
\qplmap{axioms/AxiomMxX}{atlas/figures01.pdf}{14}{4.00664pt}
\qplmap{axioms/AxiomMxX-twisted}{atlas/figures01.pdf}{15}{3.66437pt}
\qplmap{axioms/AxiomPNullB}{atlas/figures01.pdf}{16}{0pt}
\qplmap{axioms/AxiomSwap}{atlas/figures01.pdf}{17}{7.72092pt}
\qplmap{axioms/AxiomSwapDecomp}{atlas/figures01.pdf}{18}{13.96504pt}
\qplmap{axioms/AxiomSwapFixedDecomp}{atlas/figures01.pdf}{19}{13.96504pt}
\qplmap{axioms/AxiomXChangeWiresA}{atlas/figures01.pdf}{20}{23.92346pt}
\qplmap{axioms/AxiomXChangeWiresB}{atlas/figures01.pdf}{21}{24.02069pt}
\qplmap{axioms/AxiomXChangeWiresBaseA}{atlas/figures01.pdf}{22}{23.92346pt}
\qplmap{axioms/AxiomXChangeWiresBaseB}{atlas/figures01.pdf}{23}{23.92346pt}
\qplmap{axioms/AxiomXCX}{atlas/figures01.pdf}{24}{13.96504pt}
\qplmap{axioms/AxiomXCX-00}{atlas/figures01.pdf}{25}{14.15456pt}
\qplmap{axioms/AxiomXCX-01}{atlas/figures01.pdf}{26}{14.15456pt}
\qplmap{axioms/AxiomXCX-02}{atlas/figures01.pdf}{27}{14.15456pt}
\qplmap{axioms/AxiomXCX-03}{atlas/figures01.pdf}{28}{13.96504pt}
\qplmap{axioms/AxiomXCX-04}{atlas/figures01.pdf}{29}{13.96504pt}
\qplmap{axioms/AxiomXCX-05}{atlas/figures01.pdf}{30}{13.96504pt}
\qplmap{axioms/AxiomXCX-06}{atlas/figures01.pdf}{31}{13.96504pt}
\qplmap{axioms/AxiomXCX-07}{atlas/figures01.pdf}{32}{14.15456pt}
\qplmap{axioms/AxiomXCX-08}{atlas/figures01.pdf}{33}{14.15456pt}
\qplmap{axioms/AxiomXCXtop}{atlas/figures01.pdf}{34}{13.96504pt}
\qplmap{axioms/AxiomXd}{atlas/figures01.pdf}{35}{4.00664pt}
\qplmap{axioms/AxiomXd-00}{atlas/figures01.pdf}{36}{4.19615pt}
\qplmap{axioms/AxiomXd-01}{atlas/figures01.pdf}{37}{4.19615pt}
\qplmap{axioms/AxiomXMx}{atlas/figures01.pdf}{38}{4.00664pt}
\qplmap{axioms/AxiomXMx-00}{atlas/figures01.pdf}{39}{4.00664pt}
\qplmap{axioms/AxiomXMx-01}{atlas/figures01.pdf}{40}{4.19615pt}
\qplmap{axioms/AxiomXMx-twisted}{atlas/figures01.pdf}{41}{4.19615pt}
\qplmap{axioms/AxiomXX2CommA}{atlas/figures01.pdf}{42}{23.92346pt}
\qplmap{axioms/AxiomXX2CommB}{atlas/figures01.pdf}{43}{23.92346pt}
\qplmap{axioms/AxiomXXCommA}{atlas/figures01.pdf}{44}{23.92346pt}
\qplmap{axioms/AxiomXXCommB}{atlas/figures01.pdf}{45}{23.92346pt}
\qplmap{axioms/CCZCCZ-00}{atlas/figures01.pdf}{46}{42.76408pt}
\qplmap{axioms/CCZCCZ-01}{atlas/figures01.pdf}{47}{42.76408pt}
\qplmap{axioms/CCZCCZ-02}{atlas/figures01.pdf}{48}{42.76408pt}
\qplmap{axioms/CCZCCZA}{atlas/figures01.pdf}{49}{35.87378pt}
\qplmap{axioms/CCZCCZA2}{atlas/figures01.pdf}{50}{21.6474pt}
\qplmap{axioms/CCZCCZA2-00}{atlas/figures01.pdf}{51}{34.08598pt}
\qplmap{axioms/CCZCCZA2-01}{atlas/figures01.pdf}{52}{34.08598pt}
\qplmap{axioms/CCZCCZA2-02}{atlas/figures01.pdf}{53}{34.08598pt}
\qplmap{axioms/CCZCCZA2-03}{atlas/figures01.pdf}{54}{34.08598pt}
\qplmap{axioms/CCZCCZA2-04}{atlas/figures01.pdf}{55}{34.08598pt}
\qplmap{axioms/CCZCCZA2-05}{atlas/figures01.pdf}{56}{34.08598pt}
\qplmap{axioms/CCZCCZA2-06}{atlas/figures01.pdf}{57}{34.08598pt}
\qplmap{axioms/CCZCCZA2-lem}{atlas/figures01.pdf}{58}{21.28212pt}
\qplmap{axioms/CCZCCZA2-lem-00}{atlas/figures01.pdf}{59}{24.26976pt}
\qplmap{axioms/CCZCCZA2-lem-01}{atlas/figures01.pdf}{60}{24.26976pt}
\qplmap{axioms/CCZCCZA2-lem-02}{atlas/figures01.pdf}{61}{24.26976pt}
\qplmap{axioms/CCZCCZA2-lem-03}{atlas/figures01.pdf}{62}{24.26976pt}
\qplmap{axioms/CCZCCZA2-lem-04}{atlas/figures01.pdf}{63}{24.26976pt}
\qplmap{axioms/CCZCCZA2-lem-05}{atlas/figures01.pdf}{64}{24.26976pt}
\qplmap{axioms/CCZCCZA2-lem-06}{atlas/figures01.pdf}{65}{24.26976pt}
\qplmap{axioms/CCZCCZA2-lem-07}{atlas/figures01.pdf}{66}{24.26976pt}
\qplmap{axioms/CCZCCZA2-lem-08}{atlas/figures01.pdf}{67}{24.26976pt}
\qplmap{axioms/CCZCCZA2-lem-09}{atlas/figures01.pdf}{68}{24.26976pt}
\qplmap{axioms/CCZCCZA2-lem-10}{atlas/figures01.pdf}{69}{24.26976pt}
\qplmap{axioms/CCZCCZA2-lem-11}{atlas/figures01.pdf}{70}{24.26976pt}
\qplmap{axioms/CCZCCZA2-lem-12}{atlas/figures01.pdf}{71}{24.26976pt}
\qplmap{axioms/CCZCCZA2-lem-13}{atlas/figures01.pdf}{72}{24.26976pt}
\qplmap{axioms/CCZCCZA2-lem-14}{atlas/figures01.pdf}{73}{24.26976pt}
\qplmap{axioms/CCZCCZB}{atlas/figures01.pdf}{74}{35.87378pt}
\qplmap{axioms/CCZCCZB2}{atlas/figures01.pdf}{75}{21.6474pt}
\qplmap{axioms/CCZCCZB2-lem}{atlas/figures01.pdf}{76}{22.70485pt}
\qplmap{axioms/CCZCNOT}{atlas/figures01.pdf}{77}{12.68472pt}
\qplmap{axioms/CCZCNOT-00}{atlas/figures01.pdf}{78}{25.90565pt}
\qplmap{axioms/CCZCNOT-01}{atlas/figures01.pdf}{79}{25.90565pt}
\qplmap{axioms/CCZCNOT-02}{atlas/figures01.pdf}{80}{25.90565pt}
\qplmap{axioms/CCZCNOT-03}{atlas/figures01.pdf}{81}{25.90565pt}
\qplmap{axioms/CCZCNOT-04}{atlas/figures01.pdf}{82}{25.90565pt}
\qplmap{axioms/CCZCNOT-05}{atlas/figures01.pdf}{83}{25.90565pt}
\qplmap{axioms/CCZCNOT-06}{atlas/figures01.pdf}{84}{25.69226pt}
\qplmap{axioms/CCZCNOT-07}{atlas/figures01.pdf}{85}{25.69226pt}
\qplmap{axioms/CCZCNOT-08}{atlas/figures01.pdf}{86}{25.69226pt}
\qplmap{axioms/CCZCNOT-09}{atlas/figures01.pdf}{87}{26.58858pt}
\qplmap{axioms/CCZCNOT-10}{atlas/figures01.pdf}{88}{26.58858pt}
\qplmap{axioms/CCZCNOT-11}{atlas/figures01.pdf}{89}{26.58858pt}
\qplmap{axioms/CCZCNOT-12}{atlas/figures01.pdf}{90}{26.75941pt}
\qplmap{axioms/CCZCNOT-13}{atlas/figures01.pdf}{91}{26.75941pt}
\qplmap{axioms/CCZCNOT-14}{atlas/figures01.pdf}{92}{26.75941pt}
\qplmap{axioms/CCZCNOT-15}{atlas/figures01.pdf}{93}{26.75941pt}
\qplmap{axioms/CCZCNOT-17}{atlas/figures01.pdf}{94}{26.75941pt}
\qplmap{axioms/CCZCNOT-18}{atlas/figures01.pdf}{95}{26.75941pt}
\qplmap{axioms/CCZCNOT-19}{atlas/figures01.pdf}{96}{26.75941pt}
\qplmap{axioms/CCZCNOT-20}{atlas/figures01.pdf}{97}{24.89066pt}
\qplmap{axioms/CCZCNOT-21}{atlas/figures01.pdf}{98}{24.25029pt}
\qplmap{axioms/CCZCNOT-22}{atlas/figures01.pdf}{99}{24.89066pt}
\qplmap{axioms/CCZCNOT-23}{atlas/figures01.pdf}{100}{24.89066pt}
\qplmap{axioms/CCZCNOT-24}{atlas/figures02.pdf}{1}{24.89066pt}
\qplmap{axioms/CCZCNOT-25}{atlas/figures02.pdf}{2}{24.89066pt}
\qplmap{axioms/CCZCNOT-26}{atlas/figures02.pdf}{3}{24.89066pt}
\qplmap{axioms/CCZCNOT-27}{atlas/figures02.pdf}{4}{24.89066pt}
\qplmap{axioms/CCZCNOT-28}{atlas/figures02.pdf}{5}{24.89066pt}
\qplmap{axioms/CCZCNOT-29}{atlas/figures02.pdf}{6}{24.89066pt}
\qplmap{axioms/CCZCNOTbot}{atlas/figures02.pdf}{7}{25.91515pt}
\qplmap{axioms/CCZCNOTbot-00}{atlas/figures02.pdf}{8}{32.80545pt}
\qplmap{axioms/CCZCNOTbot-01}{atlas/figures02.pdf}{9}{32.80545pt}
\qplmap{axioms/CCZCNOTbot-02}{atlas/figures02.pdf}{10}{32.80545pt}
\qplmap{axioms/CCZCNOTtop}{atlas/figures02.pdf}{11}{20.93605pt}
\qplmap{axioms/CCZCS1}{atlas/figures02.pdf}{12}{25.91515pt}
\qplmap{axioms/CCZCS1-00}{atlas/figures02.pdf}{13}{25.91515pt}
\qplmap{axioms/CCZCS1-02}{atlas/figures02.pdf}{14}{25.91515pt}
\qplmap{axioms/CCZCS1-03}{atlas/figures02.pdf}{15}{25.91515pt}
\qplmap{axioms/CCZCS1-04}{atlas/figures02.pdf}{16}{25.91515pt}
\qplmap{axioms/CCZCS2}{atlas/figures02.pdf}{17}{25.91515pt}
\qplmap{axioms/CCZCS2-00}{atlas/figures02.pdf}{18}{25.91515pt}
\qplmap{axioms/CCZCS2-01}{atlas/figures02.pdf}{19}{25.91515pt}
\qplmap{axioms/CCZCS2-02}{atlas/figures02.pdf}{20}{25.91515pt}
\qplmap{axioms/CCZCS2-03}{atlas/figures02.pdf}{21}{25.91515pt}
\qplmap{axioms/CCZCS2-04}{atlas/figures02.pdf}{22}{25.91515pt}
\qplmap{axioms/CCZCS3}{atlas/figures02.pdf}{23}{13.53827pt}
\qplmap{axioms/CCZCS3-00}{atlas/figures02.pdf}{24}{25.69226pt}
\qplmap{axioms/CCZCS3-01}{atlas/figures02.pdf}{25}{25.69226pt}
\qplmap{axioms/CCZCS3-02}{atlas/figures02.pdf}{26}{25.69226pt}
\qplmap{axioms/CCZCS3-03}{atlas/figures02.pdf}{27}{25.69226pt}
\qplmap{axioms/CCZCS3-04}{atlas/figures02.pdf}{28}{25.69226pt}
\qplmap{axioms/CCZCS3-05}{atlas/figures02.pdf}{29}{25.69226pt}
\qplmap{axioms/CCZCS3-06}{atlas/figures02.pdf}{30}{25.69226pt}
\qplmap{axioms/CCZCS3-07}{atlas/figures02.pdf}{31}{25.69226pt}
\qplmap{axioms/CCZCS3-08}{atlas/figures02.pdf}{32}{25.69226pt}
\qplmap{axioms/CCZCS3-09}{atlas/figures02.pdf}{33}{25.69226pt}
\qplmap{axioms/CCZCS3-lem}{atlas/figures02.pdf}{34}{15.73384pt}
\qplmap{axioms/CCZCS3-lem-00}{atlas/figures02.pdf}{35}{15.73384pt}
\qplmap{axioms/CCZCS3-lem-01}{atlas/figures02.pdf}{36}{15.73384pt}
\qplmap{axioms/CCZCS3-lem-02}{atlas/figures02.pdf}{37}{15.73384pt}
\qplmap{axioms/CCZCS3-lem-03}{atlas/figures02.pdf}{38}{16.01843pt}
\qplmap{axioms/CCZCS3-lem-04}{atlas/figures02.pdf}{39}{15.73384pt}
\qplmap{axioms/CCZCS3-lem-05}{atlas/figures02.pdf}{40}{15.73384pt}
\qplmap{axioms/CCZCS3-lem-06}{atlas/figures02.pdf}{41}{15.73384pt}
\qplmap{axioms/CCZCS3-lem-CZ}{atlas/figures02.pdf}{42}{15.73384pt}
\qplmap{axioms/CCZCS3-lem-CZ-00}{atlas/figures02.pdf}{43}{15.81044pt}
\qplmap{axioms/CCZCS3-lem-CZ-01}{atlas/figures02.pdf}{44}{16.09503pt}
\qplmap{axioms/CCZCS3-lem-CZ-02}{atlas/figures02.pdf}{45}{15.81044pt}
\qplmap{axioms/CCZCS3-lem-CZ-03}{atlas/figures02.pdf}{46}{15.81044pt}
\qplmap{axioms/CCZCS3-lem-CZ-04}{atlas/figures02.pdf}{47}{15.81044pt}
\qplmap{axioms/CCZCS3-lem-CZ-05}{atlas/figures02.pdf}{48}{15.81044pt}
\qplmap{axioms/CCZCS3-lem-CZ-06}{atlas/figures02.pdf}{49}{15.81044pt}
\qplmap{axioms/CCZCS3-lem-CZ-07}{atlas/figures02.pdf}{50}{15.81044pt}
\qplmap{axioms/CCZCS3-lem-CZ-R}{atlas/figures02.pdf}{51}{15.73384pt}
\qplmap{axioms/CCZCS3-lem-R}{atlas/figures02.pdf}{52}{15.73384pt}
\qplmap{axioms/CCZCZ}{atlas/figures02.pdf}{53}{13.82286pt}
\qplmap{axioms/CCZCZ-00}{atlas/figures02.pdf}{54}{24.26976pt}
\qplmap{axioms/CCZCZ-01}{atlas/figures02.pdf}{55}{24.26976pt}
\qplmap{axioms/CCZCZ-02}{atlas/figures02.pdf}{56}{24.26976pt}
\qplmap{axioms/CCZCZ-03}{atlas/figures02.pdf}{57}{24.26976pt}
\qplmap{axioms/CCZCZ-04}{atlas/figures02.pdf}{58}{24.26976pt}
\qplmap{axioms/CCZCZ-05}{atlas/figures02.pdf}{59}{24.26976pt}
\qplmap{axioms/CCZCZ-06}{atlas/figures02.pdf}{60}{24.26976pt}
\qplmap{axioms/CCZCZ-07}{atlas/figures02.pdf}{61}{24.26976pt}
\qplmap{axioms/CCZCZ-08}{atlas/figures02.pdf}{62}{24.26976pt}
\qplmap{axioms/CCZCZ-09}{atlas/figures02.pdf}{63}{24.26976pt}
\qplmap{axioms/CCZCZ-10}{atlas/figures02.pdf}{64}{24.26976pt}
\qplmap{axioms/CCZCZ-11}{atlas/figures02.pdf}{65}{24.26976pt}
\qplmap{axioms/CCZCZ-12}{atlas/figures02.pdf}{66}{24.26976pt}
\qplmap{axioms/CCZCZ-13}{atlas/figures02.pdf}{67}{24.26976pt}
\qplmap{axioms/CCZCZ-14}{atlas/figures02.pdf}{68}{24.26976pt}
\qplmap{axioms/CCZCZ-15}{atlas/figures02.pdf}{69}{24.26976pt}
\qplmap{axioms/CCZCZ-16}{atlas/figures02.pdf}{70}{24.26976pt}
\qplmap{axioms/CCZCZ-17}{atlas/figures02.pdf}{71}{24.26976pt}
\qplmap{axioms/CCZCZ-18}{atlas/figures02.pdf}{72}{24.26976pt}
\qplmap{axioms/CCZCZ-19}{atlas/figures02.pdf}{73}{24.26976pt}
\qplmap{axioms/CCZCZ-20}{atlas/figures02.pdf}{74}{24.26976pt}
\qplmap{axioms/CCZCZ-21}{atlas/figures02.pdf}{75}{24.26976pt}
\qplmap{axioms/CCZCZ-22}{atlas/figures02.pdf}{76}{24.26976pt}
\qplmap{axioms/CCZCZ-23}{atlas/figures02.pdf}{77}{24.26976pt}
\qplmap{axioms/CCZCZtop}{atlas/figures02.pdf}{78}{25.91515pt}
\qplmap{axioms/CCZCZtop-00}{atlas/figures02.pdf}{79}{25.91515pt}
\qplmap{axioms/CCZCZtop-01}{atlas/figures02.pdf}{80}{25.91515pt}
\qplmap{axioms/CCZCZtop-02}{atlas/figures02.pdf}{81}{25.91515pt}
\qplmap{axioms/CCZCZtop-03}{atlas/figures02.pdf}{82}{25.91515pt}
\qplmap{axioms/CCZd-00-A}{atlas/figures02.pdf}{83}{25.77026pt}
\qplmap{axioms/CCZd-00-B}{atlas/figures02.pdf}{84}{25.69226pt}
\qplmap{axioms/CCZd-01-A}{atlas/figures02.pdf}{85}{17.67934pt}
\qplmap{axioms/CCZd-01-B}{atlas/figures02.pdf}{86}{25.69226pt}
\qplmap{axioms/CCZd-02-A}{atlas/figures02.pdf}{87}{25.69226pt}
\qplmap{axioms/CCZd-02-B}{atlas/figures02.pdf}{88}{25.69226pt}
\qplmap{axioms/CCZdef}{atlas/figures02.pdf}{89}{25.69226pt}
\qplmap{axioms/CCZdlem1}{atlas/figures02.pdf}{90}{25.69226pt}
\qplmap{axioms/CCZdlem1-00}{atlas/figures02.pdf}{91}{25.69226pt}
\qplmap{axioms/CCZdlem1-01}{atlas/figures02.pdf}{92}{25.69226pt}
\qplmap{axioms/CCZdlem1-02}{atlas/figures02.pdf}{93}{25.69226pt}
\qplmap{axioms/CCZdlem1-03}{atlas/figures02.pdf}{94}{25.69226pt}
\qplmap{axioms/CCZdlem1-04}{atlas/figures02.pdf}{95}{25.69226pt}
\qplmap{axioms/CCZdlem1-05}{atlas/figures02.pdf}{96}{25.69226pt}
\qplmap{axioms/CCZdlem1-06}{atlas/figures02.pdf}{97}{25.69226pt}
\qplmap{axioms/CCZdlem1-07}{atlas/figures02.pdf}{98}{25.69226pt}
\qplmap{axioms/CCZdlem1-08}{atlas/figures02.pdf}{99}{25.69226pt}
\qplmap{axioms/CCZdlem1-09}{atlas/figures02.pdf}{100}{25.69226pt}
\qplmap{axioms/CCZdlem1-10}{atlas/figures03.pdf}{1}{25.69226pt}
\qplmap{axioms/CCZdlem1-11}{atlas/figures03.pdf}{2}{25.69226pt}
\qplmap{axioms/CCZdlem1-12}{atlas/figures03.pdf}{3}{25.69226pt}
\qplmap{axioms/CCZdlem1-13}{atlas/figures03.pdf}{4}{25.69226pt}
\qplmap{axioms/CCZdlem1-14}{atlas/figures03.pdf}{5}{25.69226pt}
\qplmap{axioms/CCZdlem1R}{atlas/figures03.pdf}{6}{25.69226pt}
\qplmap{axioms/CCZdlem2}{atlas/figures03.pdf}{7}{25.69226pt}
\qplmap{axioms/CCZdlem2-00}{atlas/figures03.pdf}{8}{25.69226pt}
\qplmap{axioms/CCZdlem2-01}{atlas/figures03.pdf}{9}{25.69226pt}
\qplmap{axioms/CCZdlem2-02}{atlas/figures03.pdf}{10}{25.69226pt}
\qplmap{axioms/CCZdlem2-03}{atlas/figures03.pdf}{11}{25.69226pt}
\qplmap{axioms/CCZdlem2-04}{atlas/figures03.pdf}{12}{25.69226pt}
\qplmap{axioms/CCZdlem2-05}{atlas/figures03.pdf}{13}{25.69226pt}
\qplmap{axioms/CCZdlem2R}{atlas/figures03.pdf}{14}{25.69226pt}
\qplmap{axioms/CCZdlem3}{atlas/figures03.pdf}{15}{25.69226pt}
\qplmap{axioms/CCZdlem3-00}{atlas/figures03.pdf}{16}{25.69226pt}
\qplmap{axioms/CCZdlem3-01}{atlas/figures03.pdf}{17}{25.69226pt}
\qplmap{axioms/CCZdlem3-02}{atlas/figures03.pdf}{18}{25.69226pt}
\qplmap{axioms/CCZdlem3-03}{atlas/figures03.pdf}{19}{25.69226pt}
\qplmap{axioms/CCZdlem3-04}{atlas/figures03.pdf}{20}{25.69226pt}
\qplmap{axioms/CCZdlem3R}{atlas/figures03.pdf}{21}{25.69226pt}
\qplmap{axioms/CCZdlem4}{atlas/figures03.pdf}{22}{25.69226pt}
\qplmap{axioms/CCZdlem4-00}{atlas/figures03.pdf}{23}{25.69226pt}
\qplmap{axioms/CCZdlem4-01}{atlas/figures03.pdf}{24}{25.69226pt}
\qplmap{axioms/CCZdlem4-02}{atlas/figures03.pdf}{25}{25.69226pt}
\qplmap{axioms/CCZdlem4-03}{atlas/figures03.pdf}{26}{25.69226pt}
\qplmap{axioms/CCZdlem4R}{atlas/figures03.pdf}{27}{25.69226pt}
\qplmap{axioms/CCZM}{atlas/figures03.pdf}{28}{14.91513pt}
\qplmap{axioms/CCZS}{atlas/figures03.pdf}{29}{17.37946pt}
\qplmap{axioms/CCZSWAP}{atlas/figures03.pdf}{30}{17.37946pt}
\qplmap{axioms/CCZSWAP-00}{atlas/figures03.pdf}{31}{24.26976pt}
\qplmap{axioms/CCZSWAP-01}{atlas/figures03.pdf}{32}{24.26976pt}
\qplmap{axioms/CCZSWAP-02}{atlas/figures03.pdf}{33}{24.16933pt}
\qplmap{axioms/CCZSWAP-03}{atlas/figures03.pdf}{34}{24.16933pt}
\qplmap{axioms/CCZSWAP-05}{atlas/figures03.pdf}{35}{24.26976pt}
\qplmap{axioms/CCZSWAP-06}{atlas/figures03.pdf}{36}{24.26976pt}
\qplmap{axioms/CCZSWAP-07}{atlas/figures03.pdf}{37}{24.26976pt}
\qplmap{axioms/CCZSWAP-08}{atlas/figures03.pdf}{38}{24.26976pt}
\qplmap{axioms/CCZSWAP-09}{atlas/figures03.pdf}{39}{24.26976pt}
\qplmap{axioms/CCZSWAP-10}{atlas/figures03.pdf}{40}{24.26976pt}
\qplmap{axioms/CCZSWAP2}{atlas/figures03.pdf}{41}{17.37946pt}
\qplmap{axioms/CCZSWAP2-00}{atlas/figures03.pdf}{42}{24.26976pt}
\qplmap{axioms/CCZSWAP2-01}{atlas/figures03.pdf}{43}{24.26976pt}
\qplmap{axioms/CCZSWAP2-02}{atlas/figures03.pdf}{44}{24.16933pt}
\qplmap{axioms/CCZSWAP2-03}{atlas/figures03.pdf}{45}{24.16933pt}
\qplmap{axioms/CCZSWAP2-04}{atlas/figures03.pdf}{46}{24.26976pt}
\qplmap{axioms/CCZSWAP2-05}{atlas/figures03.pdf}{47}{24.26976pt}
\qplmap{axioms/CCZSWAP2-06}{atlas/figures03.pdf}{48}{24.26976pt}
\qplmap{axioms/CCZSWAP2-07}{atlas/figures03.pdf}{49}{24.26976pt}
\qplmap{axioms/CCZSWAP2-08}{atlas/figures03.pdf}{50}{24.26976pt}
\qplmap{axioms/CCZSWAP2-09}{atlas/figures03.pdf}{51}{24.26976pt}
\qplmap{axioms/CCZT}{atlas/figures03.pdf}{52}{17.37946pt}
\qplmap{axioms/CCZX}{atlas/figures03.pdf}{53}{13.82286pt}
\qplmap{axioms/CCZX-00}{atlas/figures03.pdf}{54}{25.69226pt}
\qplmap{axioms/CCZX-01}{atlas/figures03.pdf}{55}{25.76886pt}
\qplmap{axioms/CCZX-02}{atlas/figures03.pdf}{56}{25.76886pt}
\qplmap{axioms/CCZX-03}{atlas/figures03.pdf}{57}{25.76886pt}
\qplmap{axioms/CCZX-04}{atlas/figures03.pdf}{58}{25.76886pt}
\qplmap{axioms/CCZX-05}{atlas/figures03.pdf}{59}{25.76886pt}
\qplmap{axioms/CCZX-06}{atlas/figures03.pdf}{60}{25.76886pt}
\qplmap{axioms/CCZX-07}{atlas/figures03.pdf}{61}{25.76886pt}
\qplmap{axioms/CCZX-08}{atlas/figures03.pdf}{62}{25.76886pt}
\qplmap{axioms/CCZX-09}{atlas/figures03.pdf}{63}{25.76886pt}
\qplmap{axioms/CCZX-10}{atlas/figures03.pdf}{64}{25.76886pt}
\qplmap{axioms/CCZX-11}{atlas/figures03.pdf}{65}{25.76886pt}
\qplmap{axioms/CCZX-12}{atlas/figures03.pdf}{66}{25.76886pt}
\qplmap{axioms/CCZX-13}{atlas/figures03.pdf}{67}{25.76886pt}
\qplmap{axioms/CCZX-15}{atlas/figures03.pdf}{68}{25.76886pt}
\qplmap{axioms/CCZX-17}{atlas/figures03.pdf}{69}{25.76886pt}
\qplmap{axioms/CCZX-18}{atlas/figures03.pdf}{70}{25.76886pt}
\qplmap{axioms/CCZX-19}{atlas/figures03.pdf}{71}{25.76886pt}
\qplmap{axioms/CCZX-20}{atlas/figures03.pdf}{72}{25.76886pt}
\qplmap{axioms/CCZX-21}{atlas/figures03.pdf}{73}{25.76886pt}
\qplmap{axioms/CCZX-22}{atlas/figures03.pdf}{74}{25.76886pt}
\qplmap{axioms/CCZX-23}{atlas/figures03.pdf}{75}{25.76886pt}
\qplmap{axioms/CCZX-24}{atlas/figures03.pdf}{76}{25.76886pt}
\qplmap{axioms/CCZX-25}{atlas/figures03.pdf}{77}{25.76886pt}
\qplmap{axioms/CCZX-26}{atlas/figures03.pdf}{78}{25.76886pt}
\qplmap{axioms/CCZX-27}{atlas/figures03.pdf}{79}{25.76886pt}
\qplmap{axioms/CCZX-28}{atlas/figures03.pdf}{80}{25.76886pt}
\qplmap{axioms/CCZX-29}{atlas/figures03.pdf}{81}{25.76886pt}
\qplmap{axioms/CCZX-30}{atlas/figures03.pdf}{82}{25.76886pt}
\qplmap{axioms/CCZX-31}{atlas/figures03.pdf}{83}{25.76886pt}
\qplmap{axioms/CCZX-32}{atlas/figures03.pdf}{84}{25.76886pt}
\qplmap{axioms/CCZX-33}{atlas/figures03.pdf}{85}{25.69226pt}
\qplmap{axioms/CCZZ}{atlas/figures03.pdf}{86}{17.37946pt}
\qplmap{axioms/CNOTCCZ}{atlas/figures03.pdf}{87}{19.37114pt}
\qplmap{axioms/CNOTCCZbot}{atlas/figures03.pdf}{88}{25.91515pt}
\qplmap{axioms/CNOTCCZtop}{atlas/figures03.pdf}{89}{20.93605pt}
\qplmap{axioms/CNOTCS}{atlas/figures03.pdf}{90}{15.81454pt}
\qplmap{axioms/CNOTCSbot}{atlas/figures03.pdf}{91}{16.7612pt}
\qplmap{axioms/CNOTCSbot2}{atlas/figures03.pdf}{92}{19.65573pt}
\qplmap{axioms/CNOTCSrev}{atlas/figures03.pdf}{93}{15.81044pt}
\qplmap{axioms/CNOTCStop}{atlas/figures03.pdf}{94}{19.60643pt}
\qplmap{axioms/CNOTCStop-00}{atlas/figures03.pdf}{95}{24.16933pt}
\qplmap{axioms/CNOTCStop-01}{atlas/figures03.pdf}{96}{24.16933pt}
\qplmap{axioms/CNOTCStop-02}{atlas/figures03.pdf}{97}{24.16933pt}
\qplmap{axioms/CNOTCStop-03}{atlas/figures03.pdf}{98}{24.16933pt}
\qplmap{axioms/CNOTCStop2}{atlas/figures03.pdf}{99}{23.0558pt}
\qplmap{axioms/CNOTCStop2-00}{atlas/figures03.pdf}{100}{22.50096pt}
\qplmap{axioms/CNOTCStop2-01}{atlas/figures04.pdf}{1}{22.50096pt}
\qplmap{axioms/CNOTCStop2-02}{atlas/figures04.pdf}{2}{22.50096pt}
\qplmap{axioms/CNOTCStop2-03}{atlas/figures04.pdf}{3}{22.50096pt}
\qplmap{axioms/CNOTCStop2-04}{atlas/figures04.pdf}{4}{22.50096pt}
\qplmap{axioms/CNOTCZ}{atlas/figures04.pdf}{5}{13.96504pt}
\qplmap{axioms/CNOTCZbot}{atlas/figures04.pdf}{6}{13.68045pt}
\qplmap{axioms/CNOTCZtop}{atlas/figures04.pdf}{7}{17.37946pt}
\qplmap{axioms/CNOTSbot}{atlas/figures04.pdf}{8}{13.96504pt}
\qplmap{axioms/CNOTStop}{atlas/figures04.pdf}{9}{15.6334pt}
\qplmap{axioms/CNOTTbot}{atlas/figures04.pdf}{10}{13.96504pt}
\qplmap{axioms/CNOTTtop}{atlas/figures04.pdf}{11}{15.6334pt}
\qplmap{axioms/CNOTZbot}{atlas/figures04.pdf}{12}{14.20253pt}
\qplmap{axioms/CNOTZtop}{atlas/figures04.pdf}{13}{15.6334pt}
\qplmap{axioms/CSCCZ1}{atlas/figures04.pdf}{14}{25.91515pt}
\qplmap{axioms/CSCCZ2}{atlas/figures04.pdf}{15}{25.91515pt}
\qplmap{axioms/CSCCZ3}{atlas/figures04.pdf}{16}{13.53827pt}
\qplmap{axioms/CSCNOT}{atlas/figures04.pdf}{17}{15.95673pt}
\qplmap{axioms/CSCNOT-00}{atlas/figures04.pdf}{18}{17.48291pt}
\qplmap{axioms/CSCNOT-01}{atlas/figures04.pdf}{19}{17.48291pt}
\qplmap{axioms/CSCNOT-02}{atlas/figures04.pdf}{20}{17.48291pt}
\qplmap{axioms/CSCNOT-03}{atlas/figures04.pdf}{21}{17.48291pt}
\qplmap{axioms/CSCNOT-04}{atlas/figures04.pdf}{22}{17.48291pt}
\qplmap{axioms/CSCNOT-06}{atlas/figures04.pdf}{23}{17.62509pt}
\qplmap{axioms/CSCNOT-07}{atlas/figures04.pdf}{24}{17.7675pt}
\qplmap{axioms/CSCNOT-08}{atlas/figures04.pdf}{25}{17.7675pt}
\qplmap{axioms/CSCNOT-09}{atlas/figures04.pdf}{26}{16.09914pt}
\qplmap{axioms/CSCNOT-10}{atlas/figures04.pdf}{27}{16.09914pt}
\qplmap{axioms/CSCNOT-11}{atlas/figures04.pdf}{28}{16.09914pt}
\qplmap{axioms/CSCNOT-12}{atlas/figures04.pdf}{29}{16.09914pt}
\qplmap{axioms/CSCNOT-13}{atlas/figures04.pdf}{30}{16.09914pt}
\qplmap{axioms/CSCNOT-14}{atlas/figures04.pdf}{31}{16.09914pt}
\qplmap{axioms/CSCNOT-15}{atlas/figures04.pdf}{32}{16.09914pt}
\qplmap{axioms/CSCNOT-16}{atlas/figures04.pdf}{33}{16.09914pt}
\qplmap{axioms/CSCNOTbot}{atlas/figures04.pdf}{34}{16.7612pt}
\qplmap{axioms/CSCNOTbot2}{atlas/figures04.pdf}{35}{18.80196pt}
\qplmap{axioms/CSCNOTrev}{atlas/figures04.pdf}{36}{9.29222pt}
\qplmap{axioms/CSCNOTrev-00}{atlas/figures04.pdf}{37}{16.34477pt}
\qplmap{axioms/CSCNOTrev-01}{atlas/figures04.pdf}{38}{16.5218pt}
\qplmap{axioms/CSCNOTrev-02}{atlas/figures04.pdf}{39}{16.5218pt}
\qplmap{axioms/CSCNOTrev-03}{atlas/figures04.pdf}{40}{16.5218pt}
\qplmap{axioms/CSCNOTrev-04}{atlas/figures04.pdf}{41}{16.5218pt}
\qplmap{axioms/CSCNOTrev-05}{atlas/figures04.pdf}{42}{16.5218pt}
\qplmap{axioms/CSCNOTrev-06}{atlas/figures04.pdf}{43}{16.5218pt}
\qplmap{axioms/CSCNOTrev-07}{atlas/figures04.pdf}{44}{16.4452pt}
\qplmap{axioms/CSCNOTrev-08}{atlas/figures04.pdf}{45}{16.4452pt}
\qplmap{axioms/CSCNOTrev-09}{atlas/figures04.pdf}{46}{16.4452pt}
\qplmap{axioms/CSCNOTrev-10}{atlas/figures04.pdf}{47}{16.4452pt}
\qplmap{axioms/CSCNOTrev-11}{atlas/figures04.pdf}{48}{16.4452pt}
\qplmap{axioms/CSCNOTrev-12}{atlas/figures04.pdf}{49}{16.4452pt}
\qplmap{axioms/CSCNOTrev-13}{atlas/figures04.pdf}{50}{16.4452pt}
\qplmap{axioms/CSCNOTrev-14}{atlas/figures04.pdf}{51}{16.4452pt}
\qplmap{axioms/CSCNOTrev-15}{atlas/figures04.pdf}{52}{16.4452pt}
\qplmap{axioms/CSCNOTrev-16}{atlas/figures04.pdf}{53}{16.4452pt}
\qplmap{axioms/CSCNOTrev-17}{atlas/figures04.pdf}{54}{16.4452pt}
\qplmap{axioms/CSCNOTrev-18}{atlas/figures04.pdf}{55}{16.4452pt}
\qplmap{axioms/CSCNOTrev-19}{atlas/figures04.pdf}{56}{16.4452pt}
\qplmap{axioms/CSCNOTrev-20}{atlas/figures04.pdf}{57}{16.4452pt}
\qplmap{axioms/CSCNOTrev-21}{atlas/figures04.pdf}{58}{16.5218pt}
\qplmap{axioms/CSCNOTrev-22}{atlas/figures04.pdf}{59}{16.5218pt}
\qplmap{axioms/CSCNOTrev-23}{atlas/figures04.pdf}{60}{16.5218pt}
\qplmap{axioms/CSCNOTtop}{atlas/figures04.pdf}{61}{19.60643pt}
\qplmap{axioms/CSCNOTtop2}{atlas/figures04.pdf}{62}{23.0558pt}
\qplmap{axioms/CSCS-00}{atlas/figures04.pdf}{63}{24.4539pt}
\qplmap{axioms/CSCS-01}{atlas/figures04.pdf}{64}{24.4539pt}
\qplmap{axioms/CSCS-02}{atlas/figures04.pdf}{65}{24.4539pt}
\qplmap{axioms/CSCS-03}{atlas/figures04.pdf}{66}{24.4539pt}
\qplmap{axioms/CSCS2-00}{atlas/figures04.pdf}{67}{24.4539pt}
\qplmap{axioms/CSCS2-01}{atlas/figures04.pdf}{68}{19.891pt}
\qplmap{axioms/CSCS2-02}{atlas/figures04.pdf}{69}{19.891pt}
\qplmap{axioms/CSCS2-03}{atlas/figures04.pdf}{70}{19.891pt}
\qplmap{axioms/CSCS2-04}{atlas/figures04.pdf}{71}{24.4539pt}
\qplmap{axioms/CSCS3-00}{atlas/figures04.pdf}{72}{19.891pt}
\qplmap{axioms/CSCS3-01}{atlas/figures04.pdf}{73}{19.891pt}
\qplmap{axioms/CSCS3-02}{atlas/figures04.pdf}{74}{19.891pt}
\qplmap{axioms/CSCS3-03}{atlas/figures04.pdf}{75}{19.891pt}
\qplmap{axioms/CSCSA}{atlas/figures04.pdf}{76}{21.02893pt}
\qplmap{axioms/CSCSA2}{atlas/figures04.pdf}{77}{21.02893pt}
\qplmap{axioms/CSCSA3}{atlas/figures04.pdf}{78}{21.02893pt}
\qplmap{axioms/CSCSB}{atlas/figures04.pdf}{79}{21.02893pt}
\qplmap{axioms/CSCSB2}{atlas/figures04.pdf}{80}{21.02893pt}
\qplmap{axioms/CSCSB3}{atlas/figures04.pdf}{81}{21.02893pt}
\qplmap{axioms/CSCZ}{atlas/figures04.pdf}{82}{9.5056pt}
\qplmap{axioms/CSCZ-00}{atlas/figures04.pdf}{83}{15.81044pt}
\qplmap{axioms/CSCZ-01}{atlas/figures04.pdf}{84}{15.81044pt}
\qplmap{axioms/CSCZ-01b}{atlas/figures04.pdf}{85}{15.81044pt}
\qplmap{axioms/CSCZ-01c}{atlas/figures04.pdf}{86}{15.81044pt}
\qplmap{axioms/CSCZ-01d}{atlas/figures04.pdf}{87}{15.81044pt}
\qplmap{axioms/CSCZ-02}{atlas/figures04.pdf}{88}{15.81044pt}
\qplmap{axioms/CSCZ-03}{atlas/figures04.pdf}{89}{15.81044pt}
\qplmap{axioms/CSCZ-04}{atlas/figures04.pdf}{90}{15.81044pt}
\qplmap{axioms/CSCZ-05}{atlas/figures04.pdf}{91}{9.97389pt}
\qplmap{axioms/CSCZ-06}{atlas/figures04.pdf}{92}{15.6334pt}
\qplmap{axioms/CSCZ-07}{atlas/figures04.pdf}{93}{15.6334pt}
\qplmap{axioms/CSCZbot}{atlas/figures04.pdf}{94}{19.60643pt}
\qplmap{axioms/CSCZbot-00}{atlas/figures04.pdf}{95}{19.60643pt}
\qplmap{axioms/CSCZbot-01}{atlas/figures04.pdf}{96}{19.60643pt}
\qplmap{axioms/CSCZbot-02}{atlas/figures04.pdf}{97}{19.60643pt}
\qplmap{axioms/CSCZbot-03}{atlas/figures04.pdf}{98}{19.60643pt}
\qplmap{axioms/CSCZtop}{atlas/figures04.pdf}{99}{17.37946pt}
\qplmap{axioms/CSCZtop-00}{atlas/figures04.pdf}{100}{24.34636pt}
\qplmap{axioms/CSCZtop-01}{atlas/figures05.pdf}{1}{24.34636pt}
\qplmap{axioms/CSCZtop-02}{atlas/figures05.pdf}{2}{24.34636pt}
\qplmap{axioms/CSd-00-A}{atlas/figures05.pdf}{3}{9.97389pt}
\qplmap{axioms/CSd-00-B}{atlas/figures05.pdf}{4}{15.6334pt}
\qplmap{axioms/CSd-01-A}{atlas/figures05.pdf}{5}{7.72092pt}
\qplmap{axioms/CSd-01-B}{atlas/figures05.pdf}{6}{15.6334pt}
\qplmap{axioms/CSd-02-A}{atlas/figures05.pdf}{7}{7.72092pt}
\qplmap{axioms/CSd-02-B}{atlas/figures05.pdf}{8}{15.81184pt}
\qplmap{axioms/CSd-03-B}{atlas/figures05.pdf}{9}{14.15456pt}
\qplmap{axioms/CSdef}{atlas/figures05.pdf}{10}{15.6334pt}
\qplmap{axioms/CSM}{atlas/figures05.pdf}{11}{11.07051pt}
\qplmap{axioms/CSMbot}{atlas/figures05.pdf}{12}{12.20027pt}
\qplmap{axioms/CSSbot}{atlas/figures05.pdf}{13}{15.6334pt}
\qplmap{axioms/CSSC}{atlas/figures05.pdf}{14}{9.64801pt}
\qplmap{axioms/CSStop}{atlas/figures05.pdf}{15}{11.07051pt}
\qplmap{axioms/CSTbot}{atlas/figures05.pdf}{16}{15.6334pt}
\qplmap{axioms/CSTtop}{atlas/figures05.pdf}{17}{11.07051pt}
\qplmap{axioms/CSXbot}{atlas/figures05.pdf}{18}{13.96504pt}
\qplmap{axioms/CSXbot-00}{atlas/figures05.pdf}{19}{15.6334pt}
\qplmap{axioms/CSXbot-01}{atlas/figures05.pdf}{20}{15.6334pt}
\qplmap{axioms/CSXbot-02}{atlas/figures05.pdf}{21}{15.6334pt}
\qplmap{axioms/CSXbot-03}{atlas/figures05.pdf}{22}{15.6334pt}
\qplmap{axioms/CSXbot-04}{atlas/figures05.pdf}{23}{15.6334pt}
\qplmap{axioms/CSXbot-05}{atlas/figures05.pdf}{24}{15.6334pt}
\qplmap{axioms/CSXbot-06}{atlas/figures05.pdf}{25}{15.6334pt}
\qplmap{axioms/CSXbot-07}{atlas/figures05.pdf}{26}{15.6334pt}
\qplmap{axioms/CSXbot-08}{atlas/figures05.pdf}{27}{15.6334pt}
\qplmap{axioms/CSXbot-09}{atlas/figures05.pdf}{28}{15.6334pt}
\qplmap{axioms/CSXbot-09b}{atlas/figures05.pdf}{29}{15.6334pt}
\qplmap{axioms/CSXbot-10}{atlas/figures05.pdf}{30}{15.6334pt}
\qplmap{axioms/CSXbot-11}{atlas/figures05.pdf}{31}{15.6334pt}
\qplmap{axioms/CSXbot-12}{atlas/figures05.pdf}{32}{15.6334pt}
\qplmap{axioms/CSXbot-13}{atlas/figures05.pdf}{33}{15.6334pt}
\qplmap{axioms/CSXbot-14}{atlas/figures05.pdf}{34}{15.6334pt}
\qplmap{axioms/CSXbot-15}{atlas/figures05.pdf}{35}{15.6334pt}
\qplmap{axioms/CSXbot-16}{atlas/figures05.pdf}{36}{15.6334pt}
\qplmap{axioms/CSXbot-17}{atlas/figures05.pdf}{37}{13.96504pt}
\qplmap{axioms/CSXbot-18}{atlas/figures05.pdf}{38}{13.96504pt}
\qplmap{axioms/CSXbot-19}{atlas/figures05.pdf}{39}{13.96504pt}
\qplmap{axioms/CSXbot-20}{atlas/figures05.pdf}{40}{13.96504pt}
\qplmap{axioms/CSXtop}{atlas/figures05.pdf}{41}{11.07051pt}
\qplmap{axioms/CSXtop-00}{atlas/figures05.pdf}{42}{15.6334pt}
\qplmap{axioms/CSXtop-01}{atlas/figures05.pdf}{43}{15.6334pt}
\qplmap{axioms/CSXtop-02}{atlas/figures05.pdf}{44}{15.6334pt}
\qplmap{axioms/CSXtop-03}{atlas/figures05.pdf}{45}{15.6334pt}
\qplmap{axioms/CSXtop-04}{atlas/figures05.pdf}{46}{15.6334pt}
\qplmap{axioms/CSXtop-05}{atlas/figures05.pdf}{47}{15.6334pt}
\qplmap{axioms/CSXtop-06}{atlas/figures05.pdf}{48}{15.6334pt}
\qplmap{axioms/CSXtop-07}{atlas/figures05.pdf}{49}{15.6334pt}
\qplmap{axioms/CSXtop-08}{atlas/figures05.pdf}{50}{15.6334pt}
\qplmap{axioms/CSXtop-09}{atlas/figures05.pdf}{51}{15.6334pt}
\qplmap{axioms/CSXtop-10}{atlas/figures05.pdf}{52}{15.6334pt}
\qplmap{axioms/CSXtop-11}{atlas/figures05.pdf}{53}{15.6334pt}
\qplmap{axioms/CSXtop-12}{atlas/figures05.pdf}{54}{15.6334pt}
\qplmap{axioms/CSXtop-13}{atlas/figures05.pdf}{55}{15.6334pt}
\qplmap{axioms/CSXtop-14}{atlas/figures05.pdf}{56}{15.81044pt}
\qplmap{axioms/CSXtop-15}{atlas/figures05.pdf}{57}{15.6334pt}
\qplmap{axioms/CSXtop-16}{atlas/figures05.pdf}{58}{15.6334pt}
\qplmap{axioms/CSXtop-17}{atlas/figures05.pdf}{59}{15.6334pt}
\qplmap{axioms/CSXtop-18}{atlas/figures05.pdf}{60}{15.6334pt}
\qplmap{axioms/CSXtop-19}{atlas/figures05.pdf}{61}{15.81044pt}
\qplmap{axioms/CSXtop-20}{atlas/figures05.pdf}{62}{15.81044pt}
\qplmap{axioms/CSXtop-21}{atlas/figures05.pdf}{63}{15.81044pt}
\qplmap{axioms/CSXtop-22}{atlas/figures05.pdf}{64}{15.81044pt}
\qplmap{axioms/CSXtop-23}{atlas/figures05.pdf}{65}{15.81044pt}
\qplmap{axioms/CSXtop-24}{atlas/figures05.pdf}{66}{15.81044pt}
\qplmap{axioms/CSXtop-25}{atlas/figures05.pdf}{67}{15.6334pt}
\qplmap{axioms/CSXtop-26}{atlas/figures05.pdf}{68}{15.6334pt}
\qplmap{axioms/CSXtop-27}{atlas/figures05.pdf}{69}{15.6334pt}
\qplmap{axioms/CSXtop-28}{atlas/figures05.pdf}{70}{15.6334pt}
\qplmap{axioms/CSXtop-29}{atlas/figures05.pdf}{71}{15.6334pt}
\qplmap{axioms/CSXtop-30}{atlas/figures05.pdf}{72}{15.6334pt}
\qplmap{axioms/CSXtop-31}{atlas/figures05.pdf}{73}{15.6334pt}
\qplmap{axioms/CSXtop-32}{atlas/figures05.pdf}{74}{15.6334pt}
\qplmap{axioms/CSXtop-33}{atlas/figures05.pdf}{75}{15.6334pt}
\qplmap{axioms/CSXtop-34}{atlas/figures05.pdf}{76}{15.6334pt}
\qplmap{axioms/CSXtop-35}{atlas/figures05.pdf}{77}{15.6334pt}
\qplmap{axioms/CSXtop-36}{atlas/figures05.pdf}{78}{15.6334pt}
\qplmap{axioms/CSXtop-37}{atlas/figures05.pdf}{79}{15.6334pt}
\qplmap{axioms/CSXtop-38}{atlas/figures05.pdf}{80}{15.6334pt}
\qplmap{axioms/CSXtop-39}{atlas/figures05.pdf}{81}{15.6334pt}
\qplmap{axioms/CSXtop-40}{atlas/figures05.pdf}{82}{15.6334pt}
\qplmap{axioms/CSXtop-41}{atlas/figures05.pdf}{83}{15.6334pt}
\qplmap{axioms/CSXtop-42}{atlas/figures05.pdf}{84}{15.6334pt}
\qplmap{axioms/CSXtop-43}{atlas/figures05.pdf}{85}{15.6334pt}
\qplmap{axioms/CSXtop-44}{atlas/figures05.pdf}{86}{15.6334pt}
\qplmap{axioms/CSXtop-45}{atlas/figures05.pdf}{87}{15.6334pt}
\qplmap{axioms/CSXtop-46}{atlas/figures05.pdf}{88}{15.6334pt}
\qplmap{axioms/CSXtop-47}{atlas/figures05.pdf}{89}{15.6334pt}
\qplmap{axioms/CSXtop-48}{atlas/figures05.pdf}{90}{15.6334pt}
\qplmap{axioms/CSZbot}{atlas/figures05.pdf}{91}{15.6334pt}
\qplmap{axioms/CSZtop}{atlas/figures05.pdf}{92}{11.07051pt}
\qplmap{axioms/CZCCZ}{atlas/figures05.pdf}{93}{13.82286pt}
\qplmap{axioms/CZCCZtop}{atlas/figures05.pdf}{94}{25.91515pt}
\qplmap{axioms/CZCNOT}{atlas/figures05.pdf}{95}{13.96504pt}
\qplmap{axioms/CZCNOT-00}{atlas/figures05.pdf}{96}{15.81044pt}
\qplmap{axioms/CZCNOT-01}{atlas/figures05.pdf}{97}{15.81044pt}
\qplmap{axioms/CZCNOT-02}{atlas/figures05.pdf}{98}{15.81044pt}
\qplmap{axioms/CZCNOT-03}{atlas/figures05.pdf}{99}{15.81044pt}
\qplmap{axioms/CZCNOT-04}{atlas/figures05.pdf}{100}{15.81044pt}
\qplmap{axioms/CZCNOT-05}{atlas/figures06.pdf}{1}{15.81044pt}
\qplmap{axioms/CZCNOT-06}{atlas/figures06.pdf}{2}{15.6334pt}
\qplmap{axioms/CZCNOT-07}{atlas/figures06.pdf}{3}{15.6334pt}
\qplmap{axioms/CZCNOT-08}{atlas/figures06.pdf}{4}{15.81044pt}
\qplmap{axioms/CZCNOT-09}{atlas/figures06.pdf}{5}{13.96504pt}
\qplmap{axioms/CZCNOTbot}{atlas/figures06.pdf}{6}{13.68045pt}
\qplmap{axioms/CZCNOTpowL}{atlas/figures06.pdf}{7}{9.81276pt}
\qplmap{axioms/CZCNOTpowR}{atlas/figures06.pdf}{8}{15.83235pt}
\qplmap{axioms/CZCNOTpowStep-00}{atlas/figures06.pdf}{9}{9.81276pt}
\qplmap{axioms/CZCNOTpowStep-01}{atlas/figures06.pdf}{10}{15.81044pt}
\qplmap{axioms/CZCNOTpowStep-02}{atlas/figures06.pdf}{11}{15.81044pt}
\qplmap{axioms/CZCNOTpowStep-03}{atlas/figures06.pdf}{12}{15.81227pt}
\qplmap{axioms/CZCNOTtop}{atlas/figures06.pdf}{13}{17.37946pt}
\qplmap{axioms/CZCNOTtop-00}{atlas/figures06.pdf}{14}{21.87358pt}
\qplmap{axioms/CZCNOTtop-01}{atlas/figures06.pdf}{15}{21.87358pt}
\qplmap{axioms/CZCNOTtop-02}{atlas/figures06.pdf}{16}{21.87358pt}
\qplmap{axioms/CZCNOTtop-03}{atlas/figures06.pdf}{17}{21.87358pt}
\qplmap{axioms/CZCNOTtop-04}{atlas/figures06.pdf}{18}{17.37946pt}
\qplmap{axioms/CZCNOTtop-05}{atlas/figures06.pdf}{19}{17.37946pt}
\qplmap{axioms/CZCNOTtop-06}{atlas/figures06.pdf}{20}{17.37946pt}
\qplmap{axioms/CZCNOTtop-07}{atlas/figures06.pdf}{21}{17.37946pt}
\qplmap{axioms/CZCNOTtop-08}{atlas/figures06.pdf}{22}{17.37946pt}
\qplmap{axioms/CZCNOTtop-09}{atlas/figures06.pdf}{23}{21.87358pt}
\qplmap{axioms/CZCNOTtop-10}{atlas/figures06.pdf}{24}{21.87358pt}
\qplmap{axioms/CZCNOTtop-11}{atlas/figures06.pdf}{25}{21.87358pt}
\qplmap{axioms/CZCS}{atlas/figures06.pdf}{26}{9.5056pt}
\qplmap{axioms/CZCSbot}{atlas/figures06.pdf}{27}{19.60643pt}
\qplmap{axioms/CZCStop}{atlas/figures06.pdf}{28}{17.37946pt}
\qplmap{axioms/CZCZA}{atlas/figures06.pdf}{29}{17.37946pt}
\qplmap{axioms/CZCZA-00}{atlas/figures06.pdf}{30}{17.37946pt}
\qplmap{axioms/CZCZA-01}{atlas/figures06.pdf}{31}{17.37946pt}
\qplmap{axioms/CZCZA-02}{atlas/figures06.pdf}{32}{21.87358pt}
\qplmap{axioms/CZCZA-03}{atlas/figures06.pdf}{33}{22.15869pt}
\qplmap{axioms/CZCZA-04}{atlas/figures06.pdf}{34}{22.15869pt}
\qplmap{axioms/CZCZA-05}{atlas/figures06.pdf}{35}{22.15869pt}
\qplmap{axioms/CZCZA-06}{atlas/figures06.pdf}{36}{22.15869pt}
\qplmap{axioms/CZCZA-07}{atlas/figures06.pdf}{37}{21.87358pt}
\qplmap{axioms/CZCZA-08}{atlas/figures06.pdf}{38}{17.37946pt}
\qplmap{axioms/CZCZB}{atlas/figures06.pdf}{39}{17.37946pt}
\qplmap{axioms/CZd-02}{atlas/figures06.pdf}{40}{14.15456pt}
\qplmap{axioms/CZd-03}{atlas/figures06.pdf}{41}{15.88843pt}
\qplmap{axioms/CZkexp}{atlas/figures06.pdf}{42}{15.91035pt}
\qplmap{axioms/CZM}{atlas/figures06.pdf}{43}{12.20027pt}
\qplmap{axioms/CZM-00}{atlas/figures06.pdf}{44}{12.20027pt}
\qplmap{axioms/CZM-01}{atlas/figures06.pdf}{45}{15.81044pt}
\qplmap{axioms/CZM-02B}{atlas/figures06.pdf}{46}{16.59338pt}
\qplmap{axioms/CZM-03}{atlas/figures06.pdf}{47}{16.59338pt}
\qplmap{axioms/CZM-04}{atlas/figures06.pdf}{48}{16.59338pt}
\qplmap{axioms/CZnegL}{atlas/figures06.pdf}{49}{13.33766pt}
\qplmap{axioms/CZnegR}{atlas/figures06.pdf}{50}{8.84354pt}
\qplmap{axioms/CZS}{atlas/figures06.pdf}{51}{8.84354pt}
\qplmap{axioms/CZSgadgetL}{atlas/figures06.pdf}{52}{8.84354pt}
\qplmap{axioms/CZSgadgetR}{atlas/figures06.pdf}{53}{17.13405pt}
\qplmap{axioms/CZSgadgetStep-00}{atlas/figures06.pdf}{54}{16.59338pt}
\qplmap{axioms/CZSgadgetStep-01}{atlas/figures06.pdf}{55}{16.59338pt}
\qplmap{axioms/CZSgadgetStep-02}{atlas/figures06.pdf}{56}{16.59338pt}
\qplmap{axioms/CZSgadgetStep-03}{atlas/figures06.pdf}{57}{16.59338pt}
\qplmap{axioms/CZSgadgetStep-04}{atlas/figures06.pdf}{58}{16.59338pt}
\qplmap{axioms/CZSgadgetStep-IH}{atlas/figures06.pdf}{59}{8.84354pt}
\qplmap{axioms/CZsumL}{atlas/figures06.pdf}{60}{15.88843pt}
\qplmap{axioms/CZsumL-00}{atlas/figures06.pdf}{61}{15.88843pt}
\qplmap{axioms/CZsumL-01}{atlas/figures06.pdf}{62}{15.88843pt}
\qplmap{axioms/CZsumL-02}{atlas/figures06.pdf}{63}{16.13446pt}
\qplmap{axioms/CZsumL-03}{atlas/figures06.pdf}{64}{16.13446pt}
\qplmap{axioms/CZsumR}{atlas/figures06.pdf}{65}{16.13446pt}
\qplmap{axioms/CZSWAP}{atlas/figures06.pdf}{66}{5.9983pt}
\qplmap{axioms/CZSWAP-00}{atlas/figures06.pdf}{67}{15.81044pt}
\qplmap{axioms/CZSWAP-01}{atlas/figures06.pdf}{68}{15.81044pt}
\qplmap{axioms/CZSWAP-02}{atlas/figures06.pdf}{69}{15.81044pt}
\qplmap{axioms/CZT}{atlas/figures06.pdf}{70}{8.84354pt}
\qplmap{axioms/CZX}{atlas/figures06.pdf}{71}{13.96504pt}
\qplmap{axioms/CZX-00}{atlas/figures06.pdf}{72}{15.81044pt}
\qplmap{axioms/CZX-01}{atlas/figures06.pdf}{73}{15.81044pt}
\qplmap{axioms/CZX-02}{atlas/figures06.pdf}{74}{15.81044pt}
\qplmap{axioms/CZX-03}{atlas/figures06.pdf}{75}{15.81044pt}
\qplmap{axioms/CZX-04}{atlas/figures06.pdf}{76}{15.81044pt}
\qplmap{axioms/CZX-05}{atlas/figures06.pdf}{77}{15.81044pt}
\qplmap{axioms/CZX-06}{atlas/figures06.pdf}{78}{15.81044pt}
\qplmap{axioms/CZX-07}{atlas/figures06.pdf}{79}{15.81044pt}
\qplmap{axioms/CZX-08}{atlas/figures06.pdf}{80}{15.81044pt}
\qplmap{axioms/CZX-09}{atlas/figures06.pdf}{81}{15.81044pt}
\qplmap{axioms/CZX-10}{atlas/figures06.pdf}{82}{15.81044pt}
\qplmap{axioms/CZX-11}{atlas/figures06.pdf}{83}{15.81044pt}
\qplmap{axioms/CZX-12}{atlas/figures06.pdf}{84}{15.81044pt}
\qplmap{axioms/CZX-13}{atlas/figures06.pdf}{85}{15.81044pt}
\qplmap{axioms/CZZ}{atlas/figures06.pdf}{86}{8.84354pt}
\qplmap{axioms/d-cnot}{atlas/figures06.pdf}{87}{13.96504pt}
\qplmap{axioms/d-cnot-00}{atlas/figures06.pdf}{88}{14.15456pt}
\qplmap{axioms/d-cnot-01}{atlas/figures06.pdf}{89}{14.15456pt}
\qplmap{axioms/d-cnot-02}{atlas/figures06.pdf}{90}{13.62277pt}
\qplmap{axioms/GadgetCZmin}{atlas/figures06.pdf}{91}{16.09644pt}
\qplmap{axioms/GadgetCZmin-00}{atlas/figures06.pdf}{92}{15.81184pt}
\qplmap{axioms/GadgetCZmin-01}{atlas/figures06.pdf}{93}{15.81184pt}
\qplmap{axioms/GadgetCZmin-02}{atlas/figures06.pdf}{94}{15.81184pt}
\qplmap{axioms/GadgetCZmin-03}{atlas/figures06.pdf}{95}{16.16623pt}
\qplmap{axioms/GadgetCZmin-04}{atlas/figures06.pdf}{96}{16.16623pt}
\qplmap{axioms/GadgetCZmin-05}{atlas/figures06.pdf}{97}{15.81184pt}
\qplmap{axioms/GadgetCZminR}{atlas/figures06.pdf}{98}{15.81184pt}
\qplmap{axioms/MCCZ}{atlas/figures06.pdf}{99}{13.82286pt}
\qplmap{axioms/MCS}{atlas/figures06.pdf}{100}{12.76712pt}
\qplmap{axioms/MCSbot}{atlas/figures07.pdf}{1}{14.57341pt}
\qplmap{axioms/MCZ}{atlas/figures07.pdf}{2}{12.20027pt}
\qplmap{axioms/MS}{atlas/figures07.pdf}{3}{5.675pt}
\qplmap{axioms/MT}{atlas/figures07.pdf}{4}{5.675pt}
\qplmap{axioms/MZ}{atlas/figures07.pdf}{5}{5.675pt}
\qplmap{axioms/PhaseGadgetA}{atlas/figures07.pdf}{6}{15.6334pt}
\qplmap{axioms/PhaseGadgetA-00}{atlas/figures07.pdf}{7}{15.6334pt}
\qplmap{axioms/PhaseGadgetA-01}{atlas/figures07.pdf}{8}{15.6334pt}
\qplmap{axioms/PhaseGadgetA-02}{atlas/figures07.pdf}{9}{15.77582pt}
\qplmap{axioms/PhaseGadgetA-03}{atlas/figures07.pdf}{10}{14.15456pt}
\qplmap{axioms/PhaseGadgetA-04}{atlas/figures07.pdf}{11}{14.15456pt}
\qplmap{axioms/PhaseGadgetA-05}{atlas/figures07.pdf}{12}{14.15456pt}
\qplmap{axioms/PhaseGadgetB}{atlas/figures07.pdf}{13}{8.84354pt}
\qplmap{axioms/PhaseGadgetComm}{atlas/figures07.pdf}{14}{16.11244pt}
\qplmap{axioms/PhaseGadgetComm-00}{atlas/figures07.pdf}{15}{16.11244pt}
\qplmap{axioms/PhaseGadgetComm-01}{atlas/figures07.pdf}{16}{16.11244pt}
\qplmap{axioms/PhaseGadgetComm-02}{atlas/figures07.pdf}{17}{16.11244pt}
\qplmap{axioms/PhaseGadgetComm-03}{atlas/figures07.pdf}{18}{16.11244pt}
\qplmap{axioms/PhaseGadgetComm-04}{atlas/figures07.pdf}{19}{16.11244pt}
\qplmap{axioms/PhaseGadgetComm-05}{atlas/figures07.pdf}{20}{16.11244pt}
\qplmap{axioms/PhaseGadgetCommR}{atlas/figures07.pdf}{21}{16.11244pt}
\qplmap{axioms/PhaseGadgetTleftA}{atlas/figures07.pdf}{22}{15.81184pt}
\qplmap{axioms/PhaseGadgetTleftA-00}{atlas/figures07.pdf}{23}{15.81184pt}
\qplmap{axioms/PhaseGadgetTleftA-01}{atlas/figures07.pdf}{24}{15.81184pt}
\qplmap{axioms/PhaseGadgetTleftA-02}{atlas/figures07.pdf}{25}{15.95425pt}
\qplmap{axioms/PhaseGadgetTleftA-03}{atlas/figures07.pdf}{26}{14.11581pt}
\qplmap{axioms/PhaseGadgetTleftA-04}{atlas/figures07.pdf}{27}{14.11581pt}
\qplmap{axioms/PhaseGadgetTleftA-05}{atlas/figures07.pdf}{28}{14.15456pt}
\qplmap{axioms/PhaseGadgetTleftA-06}{atlas/figures07.pdf}{29}{14.29697pt}
\qplmap{axioms/PhaseGadgetTleftB}{atlas/figures07.pdf}{30}{8.98595pt}
\qplmap{axioms/SCCS}{atlas/figures07.pdf}{31}{9.64801pt}
\qplmap{axioms/SCCS-00}{atlas/figures07.pdf}{32}{15.81044pt}
\qplmap{axioms/SCCS-01}{atlas/figures07.pdf}{33}{15.81044pt}
\qplmap{axioms/SCCS-02}{atlas/figures07.pdf}{34}{15.81044pt}
\qplmap{axioms/SCCS-03}{atlas/figures07.pdf}{35}{15.81044pt}
\qplmap{axioms/SCCS-04}{atlas/figures07.pdf}{36}{15.81044pt}
\qplmap{axioms/SCCS-05}{atlas/figures07.pdf}{37}{15.81044pt}
\qplmap{axioms/SCCS-06}{atlas/figures07.pdf}{38}{15.81044pt}
\qplmap{axioms/SCCS-07}{atlas/figures07.pdf}{39}{15.81044pt}
\qplmap{axioms/SCCS-08}{atlas/figures07.pdf}{40}{15.81044pt}
\qplmap{axioms/SCCS-09}{atlas/figures07.pdf}{41}{15.81044pt}
\qplmap{axioms/SCCS-10}{atlas/figures07.pdf}{42}{15.81044pt}
\qplmap{axioms/SCCS-11}{atlas/figures07.pdf}{43}{15.81044pt}
\qplmap{axioms/SCCS-12}{atlas/figures07.pdf}{44}{15.81044pt}
\qplmap{axioms/SCCS-13}{atlas/figures07.pdf}{45}{15.81044pt}
\qplmap{axioms/SCCS-14}{atlas/figures07.pdf}{46}{15.81044pt}
\qplmap{axioms/SCCS-15}{atlas/figures07.pdf}{47}{15.81044pt}
\qplmap{axioms/SCCS-16}{atlas/figures07.pdf}{48}{15.81044pt}
\qplmap{axioms/SCCS-17}{atlas/figures07.pdf}{49}{15.81044pt}
\qplmap{axioms/SCCS-18}{atlas/figures07.pdf}{50}{15.81044pt}
\qplmap{axioms/SCCS-19}{atlas/figures07.pdf}{51}{15.81044pt}
\qplmap{axioms/SCCS-20}{atlas/figures07.pdf}{52}{15.81044pt}
\qplmap{axioms/SCCZ}{atlas/figures07.pdf}{53}{17.37946pt}
\qplmap{axioms/SCCZ-00}{atlas/figures07.pdf}{54}{25.69226pt}
\qplmap{axioms/SCCZ-01}{atlas/figures07.pdf}{55}{25.69226pt}
\qplmap{axioms/SCCZ-02}{atlas/figures07.pdf}{56}{25.69226pt}
\qplmap{axioms/SCNOTbot}{atlas/figures07.pdf}{57}{13.96504pt}
\qplmap{axioms/SCNOTtop}{atlas/figures07.pdf}{58}{15.6334pt}
\qplmap{axioms/SCNOTtop-00}{atlas/figures07.pdf}{59}{15.81044pt}
\qplmap{axioms/SCNOTtop-01}{atlas/figures07.pdf}{60}{15.6334pt}
\qplmap{axioms/SCSbot}{atlas/figures07.pdf}{61}{15.6334pt}
\qplmap{axioms/SCSbot-00}{atlas/figures07.pdf}{62}{15.6334pt}
\qplmap{axioms/SCSbot-01}{atlas/figures07.pdf}{63}{15.6334pt}
\qplmap{axioms/SCSbot-02}{atlas/figures07.pdf}{64}{15.6334pt}
\qplmap{axioms/SCSbot-03}{atlas/figures07.pdf}{65}{15.6334pt}
\qplmap{axioms/SCSbot-04}{atlas/figures07.pdf}{66}{15.6334pt}
\qplmap{axioms/SCStop}{atlas/figures07.pdf}{67}{11.07051pt}
\qplmap{axioms/SCStop-00}{atlas/figures07.pdf}{68}{15.6334pt}
\qplmap{axioms/SCStop-01}{atlas/figures07.pdf}{69}{15.6334pt}
\qplmap{axioms/SCStop-02}{atlas/figures07.pdf}{70}{15.6334pt}
\qplmap{axioms/SCStop-03}{atlas/figures07.pdf}{71}{15.6334pt}
\qplmap{axioms/SCZ}{atlas/figures07.pdf}{72}{8.84354pt}
\qplmap{axioms/SCZ-00}{atlas/figures07.pdf}{73}{15.81044pt}
\qplmap{axioms/SCZ-01}{atlas/figures07.pdf}{74}{15.81044pt}
\qplmap{axioms/Sd}{atlas/figures07.pdf}{75}{5.93002pt}
\qplmap{axioms/SM}{atlas/figures07.pdf}{76}{7.17564pt}
\qplmap{axioms/ST}{atlas/figures07.pdf}{77}{5.675pt}
\qplmap{axioms/SWAPCCZ}{atlas/figures07.pdf}{78}{17.37946pt}
\qplmap{axioms/SWAPCCZ2}{atlas/figures07.pdf}{79}{17.37946pt}
\qplmap{axioms/SWAPCZ}{atlas/figures07.pdf}{80}{5.9983pt}
\qplmap{axioms/SX}{atlas/figures07.pdf}{81}{5.675pt}
\qplmap{axioms/SZ}{atlas/figures07.pdf}{82}{5.675pt}
\qplmap{axioms/TCCZ}{atlas/figures07.pdf}{83}{17.37946pt}
\qplmap{axioms/TCCZ-00}{atlas/figures07.pdf}{84}{25.69226pt}
\qplmap{axioms/TCCZ-01}{atlas/figures07.pdf}{85}{25.69226pt}
\qplmap{axioms/TCNOTbot}{atlas/figures07.pdf}{86}{13.96504pt}
\qplmap{axioms/TCNOTtop}{atlas/figures07.pdf}{87}{15.6334pt}
\qplmap{axioms/TCNOTtop-00}{atlas/figures07.pdf}{88}{15.81044pt}
\qplmap{axioms/TCNOTtop-01}{atlas/figures07.pdf}{89}{15.81044pt}
\qplmap{axioms/TCNOTtop-02}{atlas/figures07.pdf}{90}{15.81044pt}
\qplmap{axioms/TCNOTtop-03}{atlas/figures07.pdf}{91}{15.81044pt}
\qplmap{axioms/TCNOTtop-04}{atlas/figures07.pdf}{92}{15.81044pt}
\qplmap{axioms/TCNOTtop-05}{atlas/figures07.pdf}{93}{15.81044pt}
\qplmap{axioms/TCNOTtop-06}{atlas/figures07.pdf}{94}{15.81044pt}
\qplmap{axioms/TCNOTtop-07}{atlas/figures07.pdf}{95}{15.81044pt}
\qplmap{axioms/TCNOTtop-08}{atlas/figures07.pdf}{96}{15.81044pt}
\qplmap{axioms/TCNOTtop-09}{atlas/figures07.pdf}{97}{15.81044pt}
\qplmap{axioms/TCNOTtop-10}{atlas/figures07.pdf}{98}{15.81044pt}
\qplmap{axioms/TCNOTtop-11}{atlas/figures07.pdf}{99}{15.81044pt}
\qplmap{axioms/TCNOTtop-12}{atlas/figures07.pdf}{100}{15.81044pt}
\qplmap{axioms/TCNOTtop-13}{atlas/figures08.pdf}{1}{15.81044pt}
\qplmap{axioms/TCNOTtop-14}{atlas/figures08.pdf}{2}{15.81044pt}
\qplmap{axioms/TCNOTtop-15}{atlas/figures08.pdf}{3}{15.81044pt}
\qplmap{axioms/TCNOTtop-16}{atlas/figures08.pdf}{4}{15.81044pt}
\qplmap{axioms/TCNOTtop-17}{atlas/figures08.pdf}{5}{15.81044pt}
\qplmap{axioms/TCNOTtop-18}{atlas/figures08.pdf}{6}{15.81044pt}
\qplmap{axioms/TCNOTtop-19}{atlas/figures08.pdf}{7}{15.81044pt}
\qplmap{axioms/TCNOTtop-20}{atlas/figures08.pdf}{8}{15.81044pt}
\qplmap{axioms/TCNOTtop-21}{atlas/figures08.pdf}{9}{15.81044pt}
\qplmap{axioms/TCNOTtop-22}{atlas/figures08.pdf}{10}{15.81044pt}
\qplmap{axioms/TCNOTtop-23}{atlas/figures08.pdf}{11}{15.81044pt}
\qplmap{axioms/TCNOTtop-24}{atlas/figures08.pdf}{12}{15.81044pt}
\qplmap{axioms/TCNOTtop-25}{atlas/figures08.pdf}{13}{15.81044pt}
\qplmap{axioms/TCNOTtop-26}{atlas/figures08.pdf}{14}{15.81044pt}
\qplmap{axioms/TCNOTtop-27}{atlas/figures08.pdf}{15}{15.81044pt}
\qplmap{axioms/TCNOTtop-28}{atlas/figures08.pdf}{16}{15.81044pt}
\qplmap{axioms/TCNOTtop-29}{atlas/figures08.pdf}{17}{15.81044pt}
\qplmap{axioms/TCNOTtop-30}{atlas/figures08.pdf}{18}{15.81044pt}
\qplmap{axioms/TCNOTtop-31}{atlas/figures08.pdf}{19}{15.81044pt}
\qplmap{axioms/TCNOTtop-32}{atlas/figures08.pdf}{20}{15.73384pt}
\qplmap{axioms/TCNOTtop-33}{atlas/figures08.pdf}{21}{13.96504pt}
\qplmap{axioms/TCNOTtop-34}{atlas/figures08.pdf}{22}{13.96504pt}
\qplmap{axioms/TCNOTtop-35}{atlas/figures08.pdf}{23}{13.96504pt}
\qplmap{axioms/TCNOTtop-36}{atlas/figures08.pdf}{24}{15.6334pt}
\qplmap{axioms/TCNOTtop-37}{atlas/figures08.pdf}{25}{15.6334pt}
\qplmap{axioms/TCSbot}{atlas/figures08.pdf}{26}{15.6334pt}
\qplmap{axioms/TCSbot-00}{atlas/figures08.pdf}{27}{15.6334pt}
\qplmap{axioms/TCSbot-01}{atlas/figures08.pdf}{28}{15.6334pt}
\qplmap{axioms/TCSbot-02}{atlas/figures08.pdf}{29}{15.6334pt}
\qplmap{axioms/TCSbot-03}{atlas/figures08.pdf}{30}{15.6334pt}
\qplmap{axioms/TCSbot-04}{atlas/figures08.pdf}{31}{15.6334pt}
\qplmap{axioms/TCStop}{atlas/figures08.pdf}{32}{11.07051pt}
\qplmap{axioms/TCStop-00}{atlas/figures08.pdf}{33}{15.6334pt}
\qplmap{axioms/TCStop-01}{atlas/figures08.pdf}{34}{15.6334pt}
\qplmap{axioms/TCStop-02}{atlas/figures08.pdf}{35}{15.6334pt}
\qplmap{axioms/TCStop-03}{atlas/figures08.pdf}{36}{15.6334pt}
\qplmap{axioms/TCZ}{atlas/figures08.pdf}{37}{8.84354pt}
\qplmap{axioms/TCZ-00}{atlas/figures08.pdf}{38}{15.81044pt}
\qplmap{axioms/TCZ-01}{atlas/figures08.pdf}{39}{15.81044pt}
\qplmap{axioms/TCZ-02}{atlas/figures08.pdf}{40}{15.81044pt}
\qplmap{axioms/Td}{atlas/figures08.pdf}{41}{5.85344pt}
\qplmap{axioms/TM}{atlas/figures08.pdf}{42}{7.25223pt}
\qplmap{axioms/TS}{atlas/figures08.pdf}{43}{5.675pt}
\qplmap{axioms/TX}{atlas/figures08.pdf}{44}{5.675pt}
\qplmap{axioms/TZ}{atlas/figures08.pdf}{45}{5.675pt}
\qplmap{axioms/wd}{atlas/figures08.pdf}{46}{3.93929pt}
\qplmap{axioms/XCCZ}{atlas/figures08.pdf}{47}{13.82286pt}
\qplmap{axioms/XCSbot}{atlas/figures08.pdf}{48}{13.96504pt}
\qplmap{axioms/XCStop}{atlas/figures08.pdf}{49}{15.6334pt}
\qplmap{axioms/XCZ}{atlas/figures08.pdf}{50}{13.96504pt}
\qplmap{axioms/XS}{atlas/figures08.pdf}{51}{5.675pt}
\qplmap{axioms/XT}{atlas/figures08.pdf}{52}{5.675pt}
\qplmap{axioms/XZ}{atlas/figures08.pdf}{53}{5.675pt}
\qplmap{axioms/ZCCZ}{atlas/figures08.pdf}{54}{17.37946pt}
\qplmap{axioms/ZCCZ-00}{atlas/figures08.pdf}{55}{25.69226pt}
\qplmap{axioms/ZCCZ-01}{atlas/figures08.pdf}{56}{25.69226pt}
\qplmap{axioms/ZCCZ-02}{atlas/figures08.pdf}{57}{25.69226pt}
\qplmap{axioms/ZCNOTbot}{atlas/figures08.pdf}{58}{14.20253pt}
\qplmap{axioms/ZCNOTbot-00}{atlas/figures08.pdf}{59}{15.28159pt}
\qplmap{axioms/ZCNOTbot-01}{atlas/figures08.pdf}{60}{15.28159pt}
\qplmap{axioms/ZCNOTbot-02}{atlas/figures08.pdf}{61}{15.28159pt}
\qplmap{axioms/ZCNOTbot-03}{atlas/figures08.pdf}{62}{15.28159pt}
\qplmap{axioms/ZCNOTbot-04}{atlas/figures08.pdf}{63}{15.28159pt}
\qplmap{axioms/ZCNOTbot-05}{atlas/figures08.pdf}{64}{15.28159pt}
\qplmap{axioms/ZCNOTbot-06}{atlas/figures08.pdf}{65}{15.28159pt}
\qplmap{axioms/ZCNOTbot-07}{atlas/figures08.pdf}{66}{15.28159pt}
\qplmap{axioms/ZCNOTtop}{atlas/figures08.pdf}{67}{15.6334pt}
\qplmap{axioms/ZCSbot}{atlas/figures08.pdf}{68}{15.6334pt}
\qplmap{axioms/ZCSbot-00}{atlas/figures08.pdf}{69}{15.6334pt}
\qplmap{axioms/ZCSbot-01}{atlas/figures08.pdf}{70}{15.6334pt}
\qplmap{axioms/ZCSbot-02}{atlas/figures08.pdf}{71}{15.6334pt}
\qplmap{axioms/ZCSbot-03}{atlas/figures08.pdf}{72}{15.6334pt}
\qplmap{axioms/ZCSbot-04}{atlas/figures08.pdf}{73}{15.6334pt}
\qplmap{axioms/ZCStop}{atlas/figures08.pdf}{74}{11.07051pt}
\qplmap{axioms/ZCStop-00}{atlas/figures08.pdf}{75}{15.6334pt}
\qplmap{axioms/ZCStop-01}{atlas/figures08.pdf}{76}{15.6334pt}
\qplmap{axioms/ZCStop-02}{atlas/figures08.pdf}{77}{15.6334pt}
\qplmap{axioms/ZCStop-03}{atlas/figures08.pdf}{78}{15.6334pt}
\qplmap{axioms/ZCZ}{atlas/figures08.pdf}{79}{8.84354pt}
\qplmap{axioms/ZCZ-00}{atlas/figures08.pdf}{80}{15.81044pt}
\qplmap{axioms/ZCZ-07}{atlas/figures08.pdf}{81}{15.81044pt}
\qplmap{axioms/Zd}{atlas/figures08.pdf}{82}{5.85344pt}
\qplmap{axioms/ZM}{atlas/figures08.pdf}{83}{5.675pt}
\qplmap{axioms/ZS}{atlas/figures08.pdf}{84}{5.675pt}
\qplmap{axioms/ZT}{atlas/figures08.pdf}{85}{5.675pt}
\qplmap{axioms/ZX}{atlas/figures08.pdf}{86}{5.675pt}
\qplmap{d5-transport-normalform}{atlas/figures08.pdf}{87}{17.15657pt}
\qplmap{derivations/axiom-swap-00}{atlas/figures08.pdf}{88}{13.62277pt}
\qplmap{derivations/axiom-swap-01}{atlas/figures08.pdf}{89}{14.15456pt}
\qplmap{derivations/axiom-swap-02}{atlas/figures08.pdf}{90}{13.96504pt}
\qplmap{derivations/axiom-torus-aux-00}{atlas/figures08.pdf}{91}{13.96504pt}
\qplmap{derivations/axiom-torus-aux-01}{atlas/figures08.pdf}{92}{13.96504pt}
\qplmap{derivations/axiom-torus-aux-02}{atlas/figures08.pdf}{93}{13.96504pt}
\qplmap{derivations/axiom-torus-aux-03}{atlas/figures08.pdf}{94}{13.96504pt}
\qplmap{derivations/axiom-torus-aux-04}{atlas/figures08.pdf}{95}{13.62277pt}
\qplmap{derivations/axiom-torus-aux-05}{atlas/figures08.pdf}{96}{13.62277pt}
\qplmap{derivations/axiom-torus-aux-06}{atlas/figures08.pdf}{97}{13.62277pt}
\qplmap{derivations/axiom-torus-drv-00}{atlas/figures08.pdf}{98}{13.96504pt}
\qplmap{derivations/axiom-torus-drv-01}{atlas/figures08.pdf}{99}{13.62277pt}
\qplmap{derivations/axiom-torus-drv-02}{atlas/figures08.pdf}{100}{13.62277pt}
\qplmap{derivations/axiom-torus-drv-03}{atlas/figures09.pdf}{1}{13.96504pt}
\qplmap{derivations/axiom-weyl-drv-00}{atlas/figures09.pdf}{2}{14.15456pt}
\qplmap{derivations/axiom-weyl-drv-01}{atlas/figures09.pdf}{3}{14.15456pt}
\qplmap{derivations/axiom-weyl-drv-02}{atlas/figures09.pdf}{4}{13.96504pt}
\qplmap{derivations/axiom-weyl-drv-03}{atlas/figures09.pdf}{5}{8.84354pt}
\qplmap{derivations/axiom-weyl-drv-04}{atlas/figures09.pdf}{6}{8.84354pt}
\qplmap{derivations/axiom-X-change-wires-00}{atlas/figures09.pdf}{7}{23.92346pt}
\qplmap{derivations/axiom-X-change-wires-01}{atlas/figures09.pdf}{8}{24.11298pt}
\qplmap{derivations/axiom-X-change-wires-02}{atlas/figures09.pdf}{9}{24.11298pt}
\qplmap{derivations/axiom-XX2-comm-00}{atlas/figures09.pdf}{10}{24.11298pt}
\qplmap{derivations/axiom-XX2-comm-01}{atlas/figures09.pdf}{11}{24.11298pt}
\qplmap{derivations/axiom-XX2-comm-02}{atlas/figures09.pdf}{12}{24.11298pt}
\qplmap{derivations/axiom-XX2-comm-03}{atlas/figures09.pdf}{13}{24.11298pt}
\qplmap{derivations/axiom-XX2-comm-04}{atlas/figures09.pdf}{14}{24.11298pt}
\qplmap{derivations/axiom-XX-comm-00}{atlas/figures09.pdf}{15}{24.11298pt}
\qplmap{derivations/axiom-XX-comm-01}{atlas/figures09.pdf}{16}{23.92346pt}
\qplmap{derivations/axiom-XX-comm-02}{atlas/figures09.pdf}{17}{24.11298pt}
\qplmap{derivations/axiom-XX-comm-03}{atlas/figures09.pdf}{18}{24.11298pt}
\qplmap{derivations/axiom-XX-comm-04}{atlas/figures09.pdf}{19}{23.92346pt}
\qplmap{derivations/axiom-XX-comm-05}{atlas/figures09.pdf}{20}{24.11298pt}
\qplmap{derivations/lafont-3-left}{atlas/figures09.pdf}{21}{11.11981pt}
\qplmap{derivations/lafont-3-right}{atlas/figures09.pdf}{22}{11.11981pt}
\qplmap{derivations/lafont-4-left}{atlas/figures09.pdf}{23}{11.11981pt}
\qplmap{derivations/lafont-4-right}{atlas/figures09.pdf}{24}{11.11981pt}
\qplmap{derivations/lafont-5left}{atlas/figures09.pdf}{25}{11.11981pt}
\qplmap{derivations/lafont-5right}{atlas/figures09.pdf}{26}{11.11981pt}
\qplmap{derivations/lafont-6-left}{atlas/figures09.pdf}{27}{11.47539pt}
\qplmap{derivations/lafont-6-right}{atlas/figures09.pdf}{28}{11.47539pt}
\qplmap{derivations/lafont-7-left}{atlas/figures09.pdf}{29}{18.233pt}
\qplmap{derivations/lafont-7-right}{atlas/figures09.pdf}{30}{18.233pt}
\qplmap{derivations/swapswap}{atlas/figures09.pdf}{31}{6.58278pt}
\qplmap{ladderleft}{atlas/figures09.pdf}{32}{0pt}
\qplmap{ladderright}{atlas/figures09.pdf}{33}{0pt}
\qplmap{nfaff}{atlas/figures09.pdf}{34}{0pt}
\qplmap{nfdiag}{atlas/figures09.pdf}{35}{0pt}
\qplmap{nfdiagS}{atlas/figures09.pdf}{36}{0pt}
\qplmap{nfdiagZ}{atlas/figures09.pdf}{37}{0pt}
\qplmap{pieces/CCZ}{atlas/figures09.pdf}{38}{11.00375pt}
\qplmap{pieces/CCZd}{atlas/figures09.pdf}{39}{15.53694pt}
\qplmap{pieces/CCZk}{atlas/figures09.pdf}{40}{15.39137pt}
\qplmap{pieces/CS}{atlas/figures09.pdf}{41}{8.15843pt}
\qplmap{pieces/CSd}{atlas/figures09.pdf}{42}{13.86845pt}
\qplmap{pieces/CSk}{atlas/figures09.pdf}{43}{11.02322pt}
\qplmap{pieces/CX}{atlas/figures09.pdf}{44}{11.8573pt}
\qplmap{pieces/CXk}{atlas/figures09.pdf}{45}{11.67467pt}
\qplmap{pieces/CXkminus}{atlas/figures09.pdf}{46}{11.7719pt}
\qplmap{pieces/CXkminus2}{atlas/figures09.pdf}{47}{14.71257pt}
\qplmap{pieces/CXm}{atlas/figures09.pdf}{48}{11.67467pt}
\qplmap{pieces/CZ}{atlas/figures09.pdf}{49}{6.7358pt}
\qplmap{pieces/CZd}{atlas/figures09.pdf}{50}{10.98439pt}
\qplmap{pieces/CZdef}{atlas/figures09.pdf}{51}{15.81044pt}
\qplmap{pieces/CZk}{atlas/figures09.pdf}{52}{7.9226pt}
\qplmap{pieces/empty}{atlas/figures09.pdf}{53}{4.87569pt}
\qplmap{pieces/I}{atlas/figures09.pdf}{54}{0pt}
\qplmap{pieces/M}{atlas/figures09.pdf}{55}{4.40186pt}
\qplmap{pieces/Mminus}{atlas/figures09.pdf}{56}{3.66437pt}
\qplmap{pieces/Mminus2}{atlas/figures09.pdf}{57}{3.66437pt}
\qplmap{pieces/S}{atlas/figures09.pdf}{58}{4.2pt}
\qplmap{pieces/SC}{atlas/figures09.pdf}{59}{6.7358pt}
\qplmap{pieces/Sk}{atlas/figures09.pdf}{60}{5.93002pt}
\qplmap{pieces/Skminus}{atlas/figures09.pdf}{61}{5.93002pt}
\qplmap{pieces/swap}{atlas/figures09.pdf}{62}{4.87569pt}
\qplmap{pieces/T}{atlas/figures09.pdf}{63}{4.2pt}
\qplmap{pieces/Tk}{atlas/figures09.pdf}{64}{5.85344pt}
\qplmap{pieces/Tkminus}{atlas/figures09.pdf}{65}{5.85344pt}
\qplmap{pieces/w}{atlas/figures09.pdf}{66}{3.15297pt}
\qplmap{pieces/wk}{atlas/figures09.pdf}{67}{3.93929pt}
\qplmap{pieces/wkminus}{atlas/figures09.pdf}{68}{3.93929pt}
\qplmap{pieces/X}{atlas/figures09.pdf}{69}{4.74413pt}
\qplmap{pieces/Xb1}{atlas/figures09.pdf}{70}{4.00664pt}
\qplmap{pieces/Xbn}{atlas/figures09.pdf}{71}{4.00664pt}
\qplmap{pieces/Xkminus}{atlas/figures09.pdf}{72}{4.10387pt}
\qplmap{pieces/Xkminus2}{atlas/figures09.pdf}{73}{7.04454pt}
\qplmap{pieces/Xm}{atlas/figures09.pdf}{74}{4.00664pt}
\qplmap{pieces/Z}{atlas/figures09.pdf}{75}{4.2pt}
\qplmap{pieces/Zk}{atlas/figures09.pdf}{76}{5.85344pt}
\qplmap{pieces/Zkminus}{atlas/figures09.pdf}{77}{5.85344pt}
\qplmap{Scol}{atlas/figures09.pdf}{78}{0pt}
\qplmap{Scoldef}{atlas/figures09.pdf}{79}{0pt}
\qplmap{stairleft}{atlas/figures09.pdf}{80}{0pt}
\qplmap{stairright}{atlas/figures09.pdf}{81}{0pt}
\qplmap{Tcol}{atlas/figures09.pdf}{82}{0pt}
\qplmap{Tcoldef}{atlas/figures09.pdf}{83}{0pt}
\qplmap{three-lines}{atlas/figures09.pdf}{84}{13.4116pt}
\qplmap{two-lines}{atlas/figures09.pdf}{85}{7.72092pt}
\qplmap{UCStriangleleft}{atlas/figures09.pdf}{86}{0pt}
\qplmap{UCStriangleright}{atlas/figures09.pdf}{87}{0pt}
\qplmap{USCtriangleleft}{atlas/figures09.pdf}{88}{0pt}
\qplmap{USCtriangleright}{atlas/figures09.pdf}{89}{0pt}
\qplmap{Utriangleleft}{atlas/figures09.pdf}{90}{0pt}
\qplmap{Utriangleright}{atlas/figures09.pdf}{91}{0pt}
\qplmap{Vtrapezoidleft}{atlas/figures09.pdf}{92}{0pt}
\qplmap{Vtrapezoidright}{atlas/figures09.pdf}{93}{0pt}
\qplmap{Vtriangleleft}{atlas/figures09.pdf}{94}{0pt}
\qplmap{Vtriangleright}{atlas/figures09.pdf}{95}{0pt}
\qplmap{Zcol}{atlas/figures09.pdf}{96}{0pt}
\qplmap{Zcoldef}{atlas/figures09.pdf}{97}{0pt}
\makeatother

